Generalized People Diversity: Learning a Human Perception-Aligned Diversity Representation for People Images

Capturing the diversity of people in images is challenging: recent literature tends to focus on diversifying one or two attributes, requiring expensive attribute labels or building classifiers. We introduce a diverse people image ranking method which more flexibly aligns with human notions of people diversity in a less prescriptive, label-free manner. The Perception-Aligned Text-derived Human representation Space (PATHS) aims to capture all or many relevant features of people-related diversity, and, when used as the representation space in the standard Maximal Marginal Relevance (MMR) ranking algorithm, is better able to surface a range of types of people-related diversity (e.g. disability, cultural attire). PATHS is created in two stages. First, a text-guided approach is used to extract a person-diversity representation from a pre-trained image-text model. Then this representation is fine-tuned on perception judgments from human annotators so that it captures the aspects of people-related similarity that humans find most salient. Empirical results show that the PATHS method achieves diversity better than baseline methods, according to side-by-side ratings from human annotators.

==> introduction_old.tex <==
We increasingly access and discover images through web-based recommendation and ranking systems. When such systems are queried for (and surface) photos of people, they can shape our perceptions of other people; they can reinforce or dismantle stereotypes~\cite{kay2015unequal}.
As such, there is growing interest in making these systems show more diverse and representative images of people~\cite{silva2023representation,karako2018using,celis2020implicit,noble-2018,otterbacher2018investigating}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/side_by_sides/PATHS.png}
    \caption{An example of image ranking results for the query of ``Bride'' with our proposed \ourmethodabbv method. This method promotes the images outlined in red: a bride in culturally Chinese attire, and a bride in a wheelchair.}
    \label{fig:qualitative_paths_only}
    \vspace{-20pt}
\end{figure}

``Diversity'' is a long standing goal in ranking and recommendation systems, where it is often defined as showing users a range of novel---but still relevant---query results\cite{carbonell1998use,celis2018fair}.
From a sociological perspective, ``diversity,'' is a broad term with varied definitions~\cite{plaut2015new,ashkanasy2002diversity}; here we use the term to refer to varied sociocultural identities (e.g. backgrounds, lifestyles, nationalities, religions).
Our method to ``diversify'' image sets of people hopes to align the two definitions: surfacing query-relevant images with novel perceived sociocultural identities.

Existing methods for diversifying sets of people images often suffer from a key limitation: they require a predefined list of attributes on which to diversify \cite{karako2018using,silva2023representation, TanjimGansForImageSearchDiversity}.
How we socially perceive the diversity of people, however, can be influenced by a wide range of sociocultural attributes~\cite{jackson2003recent}, such as ethnicity~\cite{rattan2013diversity}, gender expression~\cite{lindqvist2021gender}, cultural attire~\cite{reeves2012muslim,ghumman2013religious}, body shape~\cite{de2018body}, or age~\cite{kunze2011age}.
Thus, predefining a list of attributes constrains the types of diversity we can capture, and is at odds with more the complex ways people diversity is actually perceived.
Further, adding a new predefined attribute has such a high marginal cost that most work only uses one or two (typically gender and/or skin tone) \cite{celis2020implicit, TanjimGansForImageSearchDiversity}: each requires creating a new attribute classifier and integrating it into the existing system~\cite{schumann2023consensus}, as well as collecting new attribute labels for each person photographed (which can also carry ethical, legal, and privacy risks~\cite{prabhu2020large,wu2020gender}). 
Finally, using predefined attributes can perpetuate bias against non-normative images (e.g. women without long hair,  people in wheelchairs) \cite{denton2021genealogy,prabhu2020large}, or promote cultural biases from the labelling taxonomy \cite{andrews2023view, schumann2021step}.

To avoid the harms and limitations of existing people-diversity representation spaces, in this work we present \textit{\ourmethod} (PATHS), a representation space for people images that does not require the constraint of predefined people attributes.
In this new space, similarity between two images should correspond to how humans think about the diversity-relevant similarity of the two \textit{people} in the images (e.g., embeddings of the same person photographed in the office and in the park should be close together, while the embeddings of a bride in traditional Chinese clothing and a bride in traditional Korean clothing should be far apart).
We create \ourmethodabbv in two stages.
First, using a focus group, we create a broad dataset of text adjectives relevant to people diversity and use this text dataset to extract a people-diversity representation from the pre-trained CoCa image-text model \cite{wang2023concept, yu2022coca}.
Second, we use triplet metric learning methods to fine-tune this text-derived representation on the perception judgements of human annotators. We are able to do this metric learning step in a data-efficient manner, because the first text-derivation stage gives a good starting point for the representation \cite{bellet2022metric}.
The final \ourmethodabbv is a perception-aligned people-diversity representation that can be used to diversify image sets of people in a more comprehensive way.

Indeed, our results on the canonical Occupations dataset\cite{celis2020implicit}, and a new dataset we present (the Diverse People Dataset) show that \ourmethodabbv enables more comprehensive end-to-end diversity than both baselines that only use skin tone and gender signals, and visual diversity baselines that are not people-specific. On Occupations, the standard dataset for this task, \ourmethodabbv improves over baseline methods by a large margin ($57.4\%$ diversity increase). On the Diverse People Dataset, which better showcases diversification across many diversity attributes, \ourmethodabbv achieves among the best ($53.6\%$ diversity increase), yielding by far the best average performance ($55.5\%$ diversity increase) across both datasets.

Moreover, case studies demonstrate instances where \ourmethodabbv better captures the types of diversity human annotators find important: for instance, our new method most agrees with our human annotators' perception that certain cultural attire makes a person's image more different than by having different skin tone. Such nuances in perceptions of social diversity are missed by other methods.

\subsection{Contributions}
Our core contributions in this work are as follows
\begin{itemize}[leftmargin=*,noitemsep]
    \item \textbf{We develop a new method to diversify a set of images of people. Notably, this method does not require predefining a list of attributes (e.g. gender, skin tone), or training on photos labeled for such attributes.} 
    This method consists of a standard diversification algorithm applied to our new \textit{\ourmethod} (PATHS).
    \item We demonstrate empirically that  \ourmethodabbv best achieves ranking diversity on both the Occupations dataset\cite{celis2020implicit}, and the new Diverse People Dataset created for this paper.
    \item We present evidence that perceptions of diversity complex: we find that human annotators give more weight to some people-related attributes over others in diversity perception judgements;
we also present case studies where our \ourmethodabbv method---unlike other methods---agrees with human perception by correctly weighting these people-related attributes more.
    
\end{itemize}
